A Nested Partitioning Scheme for Parallel Heterogeneous Clusters

Modern supercomputers are increasingly requiring the presence of accelerators and co-processors. However, it has not been easy to achieve good performance on such heterogeneous clusters. The key challenge has been to ensure good load balance and that neither the CPU nor the accelerator is left idle. Traditional approaches have offloaded entire computations to the accelerator, resulting in an idle CPU, or have opted for task-level parallelism requiring large data transfers between the CPU and the accelerator. True work-parallelism has been hard as the Accelerators cannot directly communicate with other CPUs (besides the host) and Accelerators. In this work, we present a new nested partition scheme to overcome this problem. By partitioning the work assignment on a given node asymmetrically into boundary and interior work, and assigning the interior to the accelerator, we are able to achieve excellent efficiency while ensure proper utilization of both the CPU and Accelerator resources. The problem used for evaluating the new partition is an $hp$ discontinuous Galerkin spectral element method for a coupled elastic--acoustic wave propagation problem.

==> partition.tex <==
In order to harness the full power of Stampede, it is essential to make use of the Intel MIC co-processors. Each compute node on Stampede consists of two Intel (Sandy Bridge) Xeon CPUs, each with eight cores, and one Intel Xeon Phi (MIC) co-processor connected to the PCI bus. There are several options for making use of the MIC, both in general and in the specific case of \textit{mangll}. 

\subsection{Native Programming}
One option is to port a code entirely to the MIC, ignoring the Sandy Bridge side of the compute nodes. On-MIC parallelism can be achieved using OpenMP, and inter-node parallelism can be achieved using MPI. While native MIC applications are able to communicate directly with other MICs via Infiniband, the overhead of MIC-to-Infiniband communication without the CPU acting as a host to the MIC process is too large to make this approach feasible.

Another option is to distribute MPI processes across the Sandy Bridge cores and the MIC heterogeneously. In order to avoid MIC-to-Infiniband overhead, one must ensure that on-MIC processes only share faces with processes contained on the host compute node for that MIC. Such process-pinning, cumbersome enough on its own, quickly leads to poor load balancing.

\subsection{Offload Programming}
The most efficient option for work sharing in a large, distributed-memory application is to use offloading. In the offload model, a host process on the Sandy Bridge side of the compute node launches kernels on the MIC through offload regions. This programming mode parallels the way a GPU is used in a coprocessing environment. Offload regions can contain perform computation or data-transfer. In this model, the MIC only communicates with the host process that runs on same physical compute node. Though CPU-to-MIC memory transfer still incurs an overhead large enough to necessitate minimizing communication, the overhead is far more manageable than the MIC-to-Infiniband overhead.

In order to minimize CPU-MIC communication overhead and avoid over-scheduling the MIC, it is best to have only a single process on the CPU-side that launches offload kernels. One option, then, is to have two ``flavors'' of MPI processes, one that schedules offloading, and one that does not. Each compute node would contain several non-offload MPI processes and one MPI process that does offload. Another option is to launch one MPI-process per compute node, then have that process spawn OpenMP threads on the CPU-side as well as offload processes on the MIC side. The second option is much easier to implement under the existing \textit{mangll} framework, and much easier to load balance, and thus was the option that was implemented.

\subsection{Offload Applied to dG}
In the discontinuous Galerkin finite element method, inter-process communication consists entirely of the transfer of shared element faces. Thus, the partitioning of the global domain into processor-local domains directly controls the amount of communication required. If partitions are created such that the number of faces shared amongst processors is minimized, then communication will also be minimized. \textit{mangll} handles partitioning of the global domain by ordering elements according to the Morton ordering [ref], which forms a space-filling curve, parameterizing the elements with unique, contiguous integer IDs. This global list of elements is then spliced into roughly equally sized chunks of elements, each chunk of which is distributed to a single MPI process. While this partitioning scheme results in nearly-optimal load balancing for the pure MPI case [ref], it cannot be extended to our offloading scheme, since there is no way to limit which local domains share element faces. Partitioning must take place at two levels, then. First, the inter-node partitioning proceeds as has just been described. We assign one MPI process to each compute node, and so each MPI process owns a subdomain of adjacent elements. Next, we must partition each process' domain into elements that will be handled by the CPU and elements that will be offloaded to the MIC. 
 
There are three primary considerations in the generation of the CPU-MIC partitioning. First, we only allow interior elements (that is, elements whose faces are not shared with other compute nodes) to be offloaded to the MIC. Second, we seek to minimizing communication over the PCI bus, which is achieved by minimizing the surface area of the partition offloaded to the MIC. Third, we must consider the heterogeneous nature of load balancing between the CPU and the MIC. We expect the MIC to complete its computation in less time than the CPU for a given number of elements. The more elements the MIC owns, however, the higher the PCI communication overhead becomes. We must strike a balance between the increased compute power of the MIC and the overhead of transferring data across the PCI bus.

This approach differs significantly from the way in which a coprocessor is commonly used. A common paradigm for coprocessor computing is to offload whole computationally intensive tasks to the coprocessor. For exaxmple, in the solution of the acoustic-elastic wave equation, one might offload the \textbf{volume\_loop} to the coprocessor while the CPU computes the \textbf{int\_flux} kernel. While the \textbf{volume\_loop} kernel is certainly computationally intensive, and maps well to coprocessor architectures, the amount of data that must be transferred at each timestep is proportional to the total number of elements $K$ owned by the compute node times the number of degrees of freedom per element $(N+1)^3$. In contrast, transferring only a subset $K_{co}$ of elements to the coprocessor and transferring only shared face data, assuming that $K_{co}$ is structured such that interfacial area is minimized, is proportional to $6K^{2/3}(N+1)^2$. The tradeoff is that, although less data is transferred, we must ensure the entire timestep runs optimally on the MIC, rather than just one or two computationally-intensive kernels. 

The approach proposed in this paper is to treat the dynamic between the host and offload processes in much the same way as the dynamic between compute nodes is treated. Each host initailizes its coprocessor, then launches an offload process that runs each timestep in parallel with the host. Syncronization is only required once per time step, when the CPU and coprocessor exchange their shared face data. At the end of the computation, all of the degrees of freedom computed on the coprocessor are transferred back to the host, and so we incur the cost of transferring large datasets only once. This process is shown in Figure \ref{fig:flowchart}.

\begin{figure}

	\centering
	\includegraphics[width=\textwidth]{dgae_MIC_flowchart}
	\caption{The host-coprocessor execution flow.}
	\label{fig:flowchart}
\end{figure}

\subsection{CPU-MIC Load Balancing}
\label{sec:load_balancing}
To facilitate proper CPU-MIC load balancing, several experiments were run at different orders (N) and numbers of elements (K). For each N, K combination, execution times were recorded for each of the kernels in \textit{dgae} on both the CPU and the MIC. Additionally, memory transfer experiments between the CPU and the MIC were carried out. The time required to transfer an array of double-precision floating point numbers both to and from the MIC was observed for array sizes from 1 to 4096 megabytes (see figure \ref{fig:mic_xfer}). 

\begin{figure}[htbp]
\begin{center}
\includegraphics[width=4in]{load_balance.png}
\caption{Estimated runtimes on CPU and MIC for various load fractions. The point at which the two curves cross shows the optimal MIC work fraction for this N, K combination.}
\label{fig:micbalance}
\end{center}
\end{figure}

This data was used to produce two functions, one for the MIC $T_{MIC}(N, K)$ and one for the CPU $T_{CPU}(N, K)$, that predict the time required to process K N-th order elements for a single time step. $$T_{MIC}(N, K_{MIC}) = \sum kernel_{time,mic}(N, K_{MIC})$$ and $$T_{CPU}(N, K_{CPU}) = \sum\left[kernel_{time,cpu}(N, K_{CPU})\right] + PCI_{time}(K_{MIC})$$
$PCI_{time}(K_{MIC})$ returns an estimate of the time required to transfer shared faces between the CPU and the MIC if there are $K_{MIC}$ elements on the MIC if the surface area of the MIC partition is at a minimum.

Computation on the MIC takes place asynchronously with respect to the CPU host process. Therefore, our load balance will be optimal when $T_{MIC}=T_{CPU}$. For each N, K combination, then, we simply solve the system:

$$T_{MIC}(N, K_{MIC})=T_{CPU}(N, K_{CPU})$$
$$K=K_{MIC}+K_{CPU}$$

where $K$ is the total number of elements in a given compute-node's partition.

\begin{figure}[htbp]
\begin{center}
\includegraphics[width=4in]{data_xfer.png}
\caption{Data transfer times between CPU and MIC. Vertical bars show standard deviations in samples.}
\label{fig:mic_xfer}
\end{center}
\end{figure}

